Enhancing Autonomous Driving Safety with Collision Scenario Integration

Autonomous vehicle safety is crucial for the successful deployment of self-driving cars. However, most existing planning methods rely heavily on imitation learning, which limits their ability to leverage collision data effectively. Moreover, collecting collision or near-collision data is inherently challenging, as it involves risks and raises ethical and practical concerns. In this paper, we propose SafeFusion, a training framework to learn from collision data. Instead of over-relying on imitation learning, SafeFusion integrates safety-oriented metrics during training to enable collision avoidance learning. In addition, to address the scarcity of collision data, we propose CollisionGen, a scalable data generation pipeline to generate diverse, high-quality scenarios using natural language prompts, generative models, and rule-based filtering. Experimental results show that our approach improves planning performance in collision-prone scenarios by 56\% over previous state-of-the-art planners while maintaining effectiveness in regular driving situations. Our work provides a scalable and effective solution for advancing the safety of autonomous driving systems.

==> reviewer1.tex <==
Reviewer 14 of ICRA 2025 submission 3046

Comments to the author
======================

This paper presents a dataset and method for improving the
safety of autonomous driving algorithms. Specifically, the
Collision2k dataset is introduced, which is a dataset
consisting of 2,000 collision scenarios generated using
GPT-4. The generated data are integrated into the training
of neural planners. The experiments are conducted
thoroughly in comparison to existing methods. Overall, the
paper is well-organized and well-written. However, several
concerns prevent me from recommending it for acceptance.

(1) Limited performance on OpenScene

In the OpenScene test set, the total score of 0.832
produced by the proposed method is highlighted in bold in
Table IV. However, upon closer look, Hydra-GT achieves a
higher score, and the rule-based method PDM-closed [8]
performs even better. While the proposed method shows
higher accuracy than the other conventional methods on the
Collision2k test set, this may be due to overfitting, as
the training and test data were generated using the same
approach. Furthermore, I think reporting failure cases only
for Hydra-GT is unfair, to be published as a scientific
paper. The failure cases for Safe-Hydra should have been
included.

(2) Lack of details on data generation

I believe that utilizing GPT-4o for generating structured
representations is an interesting and somewhat novel
approach. However, the present paper provides only "a brief
example" of the prompt, lacking the reproducibility of data
generation. Furthermore, there is no analysis of how often
GPT-4o made errors, nor any comparison with human
performance. It is merely stated that the 2,000 data were
manually reviewed, but no description is given regarding
the criteria used or how quality control was conducted.

This could lead to fundamental flaws. While it may seem
unlikely, for example, it could allow the selection of a
pair of training and test sets that make the proposed
method appear superior to conventional methods. This raises
concerns that the results in Table III may be overly close
to the Hydra-GT failure cases. It is essential to clearly
describe the prompt and in-context examples provided to
GPT-4, how the generated data was cleaned, and what was
excluded. The lack of clarity in this process was a
significant concern.

Despite these weaknesses, the overall writing and
presentation quality are sufficiently high, and the
comparative experiments are also intriguing. Therefore, I
have rated the paper as a borderline paper.

Comments on the Video Attachment
================================

Video presentation was informative.

==> reviewer2.tex <==
Reviewer 18 of ICRA 2025 submission 3046

Comments to the author
======================

Summary:
The paper presents a novel approach for generating
realistic corner cases and collision scenarios for
self-driving applications. Using the generated synthetic
datasets combined with real-world data, the authors propose
to train a new planner with enhanced collision avoidance
capabilities.

Comments and concerns:
The presented approach is interesting and solves an
important problem in autonomous driving. The approach for
generating collision scenarios from language prompts
(although an existing approach) seems to have been refined
in this work. However, the core concepts of the work are
not explained clearly. Many important concepts that are
used are referenced to other work without defining them
briefly in this manuscript. This makes understanding the
formulation difficult and many statements vague. The
manuscript requires major revisions to be self-contained.
Please see the following detailed comments:

1. Clearly define or add a background (in the Introduction
or Related Work section maybe) for planning trajectory
vocabulary, multi-target knowledge distillation.

2. The contribution of detecting malicious driving
behaviors feels disjointed from the rest of the
contributions. 

3. The map region 'm', and the definition of the lane
segments must appear before the Map encoder. Currently,
they are defined just before the lane adherence compliance.


4. Please also highlight the scene decoder in Fig.2.  The
Scene Decoder section requires extensive revision. Please
define each agent's attributes in a Preliminaries section.
The mask embeddings e^{agent}_i, and e^{lane}_j are
introduced without any proper definition. Why are the
attributes modeled as a K-way Gaussian Mixture Model (not
expanded in the paper)? Since this is a core section for
collision scenario generation, the subsequent sections
become harder to follow due to its lack of clarity.

5. The authors mention discretizing a continuous action
space at the end of Page 3 without previously mentioning
how the agent's action space is assumed to be. Again, such
issues can be resolved with a dedicated background section.

6. Proper background for Hydra-MDP is required as the
current work builds on it. Without explaining its
architecture and current deficiencies, the improvements
made by Safe-Hydra cannot be fully explained. 

7. Define Maximum Mean Discrepancy.

8. The authors mention that the MMD values for speed is
better for their scenario generation than prior works. But,
Table 1 shows LCTGen performing better. The authors should
explain why this is the case.

9. Please mention the settings that are similar between
your method, TrafficGen and LCTGen that were used for
comparison.

10. The results of Tables 3 and 4 are good. They are
informative and show a good improvement.

11. The Conclusions section does not mention the method's
current limitations. 

12. The video shows a couple of collision scenarios between
two agents in intersections with several lanes. It would
have been more impressive  to see scenarios with multiple
(> 2) agents. 

I realize that the presented approach seems to require a
lot of explanations within a limited page limit. The
authors should prioritize the content to make the
manuscript  as self-contained as possible. 

Comments on the Video Attachment
================================

The video shows the trajectories used by SafeHydra and
helps highlight the its benefits over other methods.
